The strength of the interaction between quarks and gluons

Modern particle physics experiments, e.g. at the Large Hadron Collider (LHC) at CERN, crucially depend on the precise description of the scattering processes in terms of the known fundamental forces. This is limited by our current understanding of the strong nuclear force, as quantified by the strong coupling, $\alpha_s$, between quarks and gluons. Relating $\alpha_s$ to experiments poses a major challenge as the strong interactions lead to the confinement of quarks and gluons inside hadronic bound states. At high energies, however, the strong interactions become weaker ("asymptotic freedom") and thus amenable to an expansion in powers of the coupling. Attempts to relate both regimes usually rely on modeling of the bound state problem in one way or another. Using large scale numerical simulations of a first principles formulation of Quantum Chromodynamics on a space-time lattice, we have carried out a model-independent determination of $\alpha_s$ with unprecedented precision. The uncertainty, about half that of all other results combined, originates predominantly from the statistical Monte Carlo evaluation and has a clear probabilistic interpretation. The result for $\alpha_s$ describes a variety of physical phenomena over a wide range of energy scales. If used as input information, it will enable significantly improved analyses of many high energy experiments, by removing an important source of theoretical uncertainty. This will increase the likelihood to uncover small effects of yet unknown physics, and enable stringent precision tests of the Standard Model. In summary, this result boosts the discovery potential of the LHC and future colliders, and the methods developed in this work pave the way for even higher precision in the future.

==> table_bg_shifts.tex <==

| 5.029(33) | 5.248(28) | 5.344(22) | 5.469(31) | 5.646(39) | 5.740(51) |
| 5.030(33) | 5.253(28) | 5.346(22) | 5.474(31) | 5.658(39) | 5.760(51) |
| 5.031(33) | 5.257(28) | 5.348(22) | 5.479(31) | 5.670(39) | 5.779(51) |
| 5.032(33) | 5.262(28) | 5.349(22) | 5.484(31) | 5.682(39) | 5.799(51) |





